Adaptation Speed Analysis for Fairness-aware Causal Models

For example, in machine translation tasks, to achieve bidirectional translation between two languages, the source corpus is often used as the target corpus, which involves the training of two models with opposite directions. The question of which one can adapt most quickly to a domain shift is of significant importance in many fields. Specifically, consider an original distribution p that changes due to an unknown intervention, resulting in a modified distribution p*. In aligning p with p*, several factors can affect the adaptation rate, including the causal dependencies between variables in p. In real-life scenarios, however, we have to consider the fairness of the training process, and it is particularly crucial to involve a sensitive variable (bias) present between a cause and an effect variable. To explore this scenario, we examine a simple structural causal model (SCM) with a cause-bias-effect structure, where variable A acts as a sensitive variable between cause (X) and effect (Y). The two models, respectively, exhibit consistent and contrary cause-effect directions in the cause-bias-effect SCM. After conducting unknown interventions on variables within the SCM, we can simulate some kinds of domain shifts for analysis. We then compare the adaptation speeds of two models across four shift scenarios. Additionally, we prove the connection between the adaptation speeds of the two models across all interventions.

==> fig.tex <==
\begin{figure*}[htbp]
    \centering
    \subfigure[Confounder,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/scatter_dense_A_k=20.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_1500/scatter_dense_A_k=20.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/curves_dense_A_k=20.pdf}
    \end{minipage}
    }%2

\centering
    \subfigure[Cause,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/scatter_dense_X_k=20.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Cause,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_1500/scatter_dense_X_k=20.pdf}
    \end{minipage}%
    }%
    \subfigure[Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/curves_dense_X_k=20.pdf}
    \end{minipage}
    }%2

    \centering
    \subfigure[Confounder and Cause,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/scatter_dense_AandX_k=20.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_1500/scatter_dense_AandX_k=20.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/curves_dense_AandX_k=20.pdf}
    \end{minipage}
    }%2

        \centering
    \subfigure[Effect,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/scatter_dense_Y_k=20.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Effect,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_1500/scatter_dense_Y_k=20.pdf}
    \end{minipage}%
    }%
    \subfigure[Effect]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/synthetic_500/curves_dense_Y_k=20.pdf}
    \end{minipage}
    }%2
    
    \centering
    \caption{\textbf{Results on synthetic data.} The scatter plots of the first column are showing the positive relation between the KL-divergence after one quarter of training terms, whlie the second column are showing the relation after three quarters of training terms. For each point, the bule point represent a pair $(p^{(0)},p^*)$ in causal model while the red point represent that in anticausl model. The curve in the third column describes the relative relationship between the speeds of the two models. The shadow shows the (5,95) percentiles of the KL-divergence. Here we set $K_{synthetic}$=20. }
    \label{fig:synthetic result}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%mnist data
\begin{figure*}[htbp]
    \centering
    \subfigure[Confounder,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/scatter_dense_A_k=10.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_1500/scatter_dense_A_k=10.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/curves_dense_A_k=10.pdf}
    \end{minipage}
    }%2

\centering
    \subfigure[Cause,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/scatter_dense_X_k=10.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Cause,T=1500]{ 
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_1500/scatter_dense_X_k=10.pdf}
    \end{minipage}%
    }%
    \subfigure[Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/curves_dense_X_k=10.pdf}
    \end{minipage}
    }%2

    \centering
    \subfigure[Confounder and Cause,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/scatter_dense_AandX_k=10.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_1500/scatter_dense_AandX_k=10.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/curves_dense_AandX_k=10.pdf}
    \end{minipage}
    }%2

        \centering
    \subfigure[Effect,T=500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/scatter_dense_Y_k=10.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Effect,T=1500]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_1500/scatter_dense_Y_k=10.pdf}
    \end{minipage}%
    }%
    \subfigure[Effect]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/mnist_500/curves_dense_Y_k=10.pdf}
    \end{minipage}
    }%2
    
    \centering
    \caption{\textbf{Results on mnist data.} The relations between the convergence speed of the two models is consistent with previous experiments on synthetic data. Here we set $K_{MNIST}=10$}.
    \label{fig:mnist result}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%adult data
\item \textbf{Adult} 
    Beside multiple categorical variables, we want to look at the results on the dichotomous variables. As shown in the (Fig.~\ref{fig:adult result}) below, the convergence rate of both models is accelerated. The speed relationship of the causal model and the anticausal model is the same as the results in the previous two experiments, but the two curves are much closer together.
\begin{figure*}[htbp]
    \centering
    \subfigure[Confounder,T=50]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_50/scatter_dense_A_k=2.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder,T=150]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/scatter_dense_A_k=2.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/curves_dense_A_k=2.pdf}
    \end{minipage}
    }%2

\centering
    \subfigure[Cause,T=50]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_50/scatter_dense_X_k=2.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Cause,T=150]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/scatter_dense_X_k=2.pdf}
    \end{minipage}%
    }%
    \subfigure[Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/curves_dense_X_k=2.pdf}
    \end{minipage}
    }%2

    \centering
    \subfigure[Confounder and Cause,T=50]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_50/scatter_dense_AandX_k=2.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause,T=150]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/scatter_dense_AandX_k=2.pdf}
    \end{minipage}%
    }%
    \subfigure[Confounder and Cause]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/curves_dense_AandX_k=2.pdf}
    \end{minipage}
    }%2

        \centering
    \subfigure[Effect,T=50]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_50/scatter_dense_Y_k=2.pdf}
%\caption{fig1}
    \end{minipage}%
    }%
    \subfigure[Effect,T=150]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/scatter_dense_Y_k=2.pdf}
    \end{minipage}%
    }%
    \subfigure[Effect]{
    \begin{minipage}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=2in]{img/adult_150/curves_dense_Y_k=2.pdf}
    \end{minipage}
    }%2
    
    \centering
    \caption{\textbf{Results on adult data.} As an experiment using binary variables, both the causal and the anticausal model converge more faster with the relation in the two previous experiments. Further, two adaptation curves are closer with $K_{Adult}=2$.}
    \label{table:adult result}
\end{itemize}

